Harmonic Stability Analysis of Microgrids with Converter-Interfaced Distributed Energy Resources, Part II: Case Studies

In Part I of this paper a method for the Harmonic Stability Assessment (HSA) of power systems with a high share of Converter-Interfaced Distributed Energy Resources (CIDERs) was proposed. Specifically, the Harmonic State-Space (HSS) model of a generic power system is derived through combination of the components HSS models. The HSS models of CIDERs and grid are based on Linear Time-Periodic (LTP) models, capable of representing the coupling between different harmonics. In Part II, the HSA of a grid-forming, and two grid-following CIDERs (i.e., ex- and including the DC-side modelling) is performed. More precisely, the classification of the eigenvalues, the impact of the maximum harmonic order on the locations of the eigenvalues, and the sensitivity curves of the eigenvalues w.r.t. to control parameters are provided. These analyses allow to study the physical meaning and origin of the CIDERs eigenvalues. Additionally, the HSA is performed for a representative example system derived from the CIGRE low-voltage benchmark system. A case of harmonic instability is identified through the system eigenvalues, and validated with Time-Domain Simulations (TDS) in Simulink. It is demonstrated that, as opposed to stability analyses based on Linear Time-Invariant (LTI) models, the HSA is suitable for the detection of harmonic instability.

==> Figures/Resource_Model.tex <==
{

\tikzstyle{system}=[rectangle, draw=black, minimum width=4.0cm, minimum height=1.0cm, inner sep=0pt]
\tikzstyle{block}=[rectangle, draw=black, minimum size=0.8cm, inner sep=0pt]
\tikzstyle{dot}=[circle, draw=black, fill=black, minimum size=0.1cm, inner sep=0pt]

\tikzstyle{signal}=[-latex]%,thick

\scriptsize

\begin{tikzpicture}

	\def\dx{1.0}
	\def\dy{1.0}
	
	%	++++++++++
	
	%	Converter
	
	\node[system] (P) at (0,1.2*\dy)
	{%
	$
	\begin{aligned}
		    \dot{\mathbf{x}}_{\pwr}
		&=      \mathbf{A}_{\pwr}\mathbf{x}_{\pwr}
		    +   \mathbf{B}_{\pwr}\mathbf{u}_{\pwr}
		    +   \mathbf{E}_{\pwr}\mathbf{w}_{\pwr}
	    \\
		    \mathbf{y}_{\pwr}
		&=      \mathbf{C}_{\pwr}\mathbf{x}_{\pwr}
		    +   \mathbf{D}_{\pwr}\mathbf{u}_{\pwr}
		    +   \mathbf{F}_{\pwr}\mathbf{w}_{\pwr}
	\end{aligned}
	$
	};
	
	\node at ($(P.north)+(0,0.3*\dy)$) {Power Hardware $\pwr$};
	
	\node[system] (C) at (0,-1.2*\dy)
	{%
	$
	\begin{aligned}
		    \dot{\mathbf{x}}_{\ctrl}
		&=      \mathbf{A}_{\ctrl}\mathbf{x}_{\ctrl}
		    +   \mathbf{B}_{\ctrl}\mathbf{u}_{\ctrl}
		    +   \mathbf{E}_{\ctrl}\mathbf{w}_{\ctrl}
	    \\
		    \mathbf{y}_{\ctrl}
		&=      \mathbf{C}_{\ctrl}\mathbf{x}_{\ctrl}
		    +   \mathbf{D}_{\ctrl}\mathbf{u}_{\ctrl}
		    +   \mathbf{F}_{\ctrl}\mathbf{w}_{\ctrl}
	\end{aligned}
	$
	};
	
	\node at ($(C.north)+(0,0.3*\dy)$) {Control Software $\ctrl$};
	
	\node[block] (TPC) at ($0.5*(P.east)+0.5*(C.east)+(0.4*\dx,0)$) {$\mathbf{T}_{\ctrl|\pwr}$};
	\node[block] (TCP) at ($0.5*(P.west)+0.5*(C.west)-(0.4*\dx,0)$) {$\mathbf{T}_{\pwr|\ctrl}$};
	
	\node[dot] (YP) at ($(P.east)+(0.4*\dx,0)$) {};
	
	\draw[-] (P.east) to (YP.west);
	\draw[signal] (YP.south) to node[right]{$\mathbf{y}_{\pwr,\lambda}$} (TPC.north);
	\draw[signal] (TPC.south)
		to node[right]{$\mathbf{u}_{\ctrl,\lambda}$} ($(C.east)+(0.4*\dx,0.3*\dy)$)
		to ($(C.east)+(0,0.3*\dy)$);
	
	\draw[signal] (C.west)
		to ($(C.west)-(0.4*\dx,0)$)
		to node[left]{$\mathbf{y}_{\ctrl}$} ($(TCP.south)$);
	\draw[signal] (TCP.north)
		to node[left]{$\mathbf{u}_{\pwr}$} ($(P.west)-(0.4*\dx,0.3*\dy)$)
		to ($(P.west)-(0,0.3*\dy)$);
		
	%	++++++++++
	
	%	Grid
	\node[block] (TPR) at ($(TPC)+(\dx,0)$) {$\mathbf{T}_{\ctrl|\pwr}$};
	\node[dot] (WP) at ($(TPR)+(0,2.4*\dy)$) {};
	\node[block] (TGP1) at ($(WP)+(\dx,0)$) {$\mathbf{T}_{\pwr|\grd}$};
	\node[block] (TGP2) at ($(TGP1)-(0,1.2*\dy)$) {$\mathbf{T}_{\grd|\pwr}$};
	\node (WG) at ($(TGP1)+(1.2*\dx,0)$) {$\mathbf{w}_{\grd}$};
	\node (YG) at ($(TGP2)+(1.2*\dx,0)$) {$\mathbf{y}_{\grd}$};
	
	\draw[signal] (WG.west) to (TGP1.east);
	\draw[signal] (TGP2.east) to (YG.west);
	\draw[-] (TGP1.west) to node[near end,above]{$\mathbf{w}_{\pwr}$} (WP.east) ;
	\draw[signal] (WP.south) to (TPR.north);
	\draw[signal] (WP.west)
		to ($(P.west)+(-0.4*\dx,1.2*\dy)$)
		to ($(P.west)+(-0.4*\dx,0.3*\dy)$)
		to ($(P.west)+(0,0.3*\dy)$);
	\draw[signal] (YP.east) to node[near start,above]{$\mathbf{y}_{\pwr,\Lambda}$} (TGP2.west);
	
	\node at ($0.5*(WG)+0.5*(YG)$) {Grid $\grd$};
	
	%	++++++++++
	
	%	Reference
	
	\node[block] (R) at ($(TPR)-(0,1.5*\dy)$) {$\mathbf{r}(\cdot,\cdot)$};
	\node (SP) at ($(R)+1.7*(\dx,0)$) {$\mathbf{w}_{\spt}$};
	
	\draw[signal] (SP.west) to (R.east);
	\draw[signal] (TPR.south) to node[right]{$\mathbf{w}_{\refr}$} (R.north);
	\draw[signal] (R.west) to node[above]{$\mathbf{w}_{\ctrl}$} ($(C.east)-(0,0.3*\dy)$);
	
	\node at ($(SP)+0.4*(0,\dy)$) {Setpoint $\spt$};
	
\end{tikzpicture}

}

==> Figures/ciders/resource_state_vector.tex <==
{
	\tikzstyle{square}=[rectangle,minimum height=0.75cm,minimum width=1cm,inner sep=0mm]
	\tikzstyle{UG1}=[]
	\tikzstyle{UG3}=[dashed]
	\tikzstyle{signalP}=[-latex,color2]
	\tikzstyle{signalN}=[-latex,color3]
	\tikzstyle{signalH}=[-latex,color4]
	
	\begin{circuitikz}
		\scriptsize
		
		\def\BlockSize{1.0}	% 1.2
		\def\X{3}	% 3.2
		\def\Y{3}	% 3.0
		\def\dlX{0.5}
		\def\dlY{0.75}
		\def\dload{0.4}
		
		% ===================================================
		
		% PH
		\node[square] (PQ1phm1) at (0,0) {$\mathbf{X}_{\pwr,-1}$};
		\draw[UG1,gray] (PQ1phm1.south west) to (PQ1phm1.south east);
		\node[square] (PQ1ph0) at ($(PQ1phm1)-(0,\dlY)$) {$\mathbf{X}_{\pwr,0}$};
		\draw[UG1,gray] (PQ1ph0.south west) to (PQ1ph0.south east);
		\node[square] (PQ1php1) at ($(PQ1ph0)-(0,\dlY)$) {$\mathbf{X}_{\pwr,+1}$};
		% brace	
		\draw [decorate,decoration={brace,amplitude=4pt,mirror,raise=1pt},yshift=0pt]
		(PQ1phm1.north west) -- (PQ1php1.south west) node [black,midway,xshift=-0.4cm] {$\hat{\mathbf{X}}_{\pwr}$};
%		\draw [decorate,white,decoration={brace,amplitude=4pt,raise=1pt},yshift=0pt]
%		(PQ1phm1.north east) -- (PQ1php1.south east) node [white,midway,xshift=0.4cm] {$\hat{\mathbf{X}}_{\pwr}$};
		
		% draw outer box
		\draw[UG1,black] (PQ1php1.south west) to (PQ1php1.south east);
		\draw[UG1,black] (PQ1phm1.north east) to (PQ1php1.south east);
		\draw[UG1,black] (PQ1phm1.north west) to (PQ1phm1.north east);
		\draw[UG1,black] (PQ1phm1.north west) to (PQ1php1.south west);
		
		% ===================================================
		% CS
		\node[square] (PQ1csm2) at ($(PQ1php1)-(0,0.08*\dlY)-(0,\dlY)$) {$\mathbf{X}_{\ctrl, -2}$};
		\draw[UG1,gray] (PQ1csm2.south west) to (PQ1csm2.south east);
		\node[square] (PQ1csm1) at ($(PQ1csm2)-(0,\dlY)$) {$\mathbf{X}_{\ctrl,-1}$};
		\draw[UG1,gray] (PQ1csm1.south west) to (PQ1csm1.south east);
		\node[square] (PQ1cs0) at ($(PQ1csm1)-(0,\dlY)$) {$\mathbf{X}_{\ctrl,0}$};
		\draw[UG1,gray] (PQ1cs0.south west) to (PQ1cs0.south east);
		\node[square] (PQ1csp1) at ($(PQ1cs0)-(0,\dlY)$) {$\mathbf{X}_{\ctrl,+1}$};
		\draw[UG1,gray] (PQ1csp1.south west) to (PQ1csp1.south east);
		\node[square] (PQ1csp2) at ($(PQ1csp1)-(0,\dlY)$) {$\mathbf{X}_{\ctrl,+2}$};
		% brace
		\draw [decorate,decoration={brace,amplitude=4pt,mirror,raise=1pt},yshift=0pt]
		(PQ1csm2.north west) -- (PQ1csp2.south west) node [black,midway,xshift=-0.4cm] {$\hat{\mathbf{X}}_{\ctrl}$};
		
		% draw outer box
		\draw[UG1,black] (PQ1csp2.south west) to (PQ1csp2.south east);
		\draw[UG1,black] (PQ1csm2.north east) to (PQ1csp2.south east);
		\draw[UG1,black] (PQ1csm2.north west) to (PQ1csm2.north east);
		\draw[UG1,black] (PQ1csm2.north west) to (PQ1csp2.south west);

		
		%		\node (T1) at ($(\X/2,5*\dlY)$) {$\phsABC$ to $\cmpDQZ$ Transformation:};
		
		
	\end{circuitikz}
}

==> Figures/systems/system_state_vector.tex <==
{
	\tikzstyle{square}=[rectangle,draw=black,minimum height=0.5cm,minimum width=0.5cm,inner sep=0mm]
	\tikzstyle{UG1}=[]
	\tikzstyle{UG3}=[dashed]
	\tikzstyle{signalP}=[-latex,color2]
	\tikzstyle{signalN}=[-latex,color3]
	\tikzstyle{signalH}=[-latex,color4]
	
	\begin{circuitikz}
		\scriptsize
		
		\def\BlockSize{1.0}	% 1.2
		\def\X{3}	% 3.2
		\def\Y{0.65}	% 3.0
		\def\dlX{0.5}
		\def\dlY{0.039}
		\def\hTE{20}%9}
		\def\hPQ{57}
		\def\hG{81}
		
		% ===================================================
		% resources
		
		% Resources
		\node[square,minimum height=\hTE*\dlY cm,label={[rotate=90]center:$\hat{\mathbf{X}}_{\TE}$}] (TE) at ($(0,0)$) {};
		\node[square,minimum height=\hPQ*\dlY cm,label={[rotate=90]center:$\hat{\mathbf{X}}_{\mathrm{PQ},1}$}] (PQ1) at ($(TE)-\hPQ*\dlY*0.5*(0,1)-\hTE*\dlY*0.5*(0,1)$) {};
		\node[square,minimum height=\hPQ*\dlY cm,label={[rotate=90]center:$\hat{\mathbf{X}}_{\mathrm{PQ},2}$}] (PQ2) at ($(PQ1)-(0,\hPQ*\dlY)$) {};
		
		% grid
		\node[square,minimum height=\hG*\dlY cm,label={[rotate=90]center:$\hat{\mathbf{X}}_{\Grd,1}$}] (G) at ($(PQ2)-\hPQ*\dlY*0.5*(0,1)-\hG*\dlY*0.5*(0,1)$) {};
		
		% PQ2
		
		
		% ===================================================
		% grid
		
		
		\node (T) at ($(G.south)-(0,\Y)$) {%
			\begin{tabular}{c}
				System State Vector\\
				$\hat{\mathbf{X}}_{\Prc}$
			\end{tabular}
		};
		
		
	\end{circuitikz}
}

==> Sections/Biographies.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/Author/jkmb}}]{Johanna Kristin Maria Becker}
	(S’19) received the B.Sc. degree in Microsystems Engineering from Freiburg University, Germany in 2015 and the M.Sc. degree in Electrical Engineering from the Swiss Federal Institute of Technology of Lausanne (EPFL), Lausanne, Switzerland in 2019.
	%
    She is currently pursuing a Ph.D. degree at the Distributed Electrical System Laboratory, EPFL, with a focus on robust control and stability assessment of active distribution systems in presence of harmonics.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/Author/amk}}]{Andreas Martin Kettner}
	(S’15-M’19) received the M.Sc. degree in electrical engineering and information technology from the Swiss Federal Institute of Technology of Zürich (ETHZ), Zürich, Switzerland in 2014, and the Ph.D. degree in power systems engineering from the Swiss Federal Institute of Technology of Lausanne (EPFL), Lausanne, Switzerland in 2019.
	He was a postdoctoral researcher at the Distributed Electrical Systems Laboratory (DESL) of EPFL from 2019 to 2020.
	Since then, he has been working as a project engineer for PSI NEPLAN AG in K{\"u}snacht, Switzerland and continues to collaborate with DESL.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/Author/mp}}]{Mario Paolone}
	(M’07–SM’10-F'22) received the M.Sc. (Hons.) and Ph.D. degrees in electrical engineering from the University of Bologna, Italy, in 1998 and 2002. 
    From 2005 to 2011, he was an Assistant Professor in power systems with the University of Bologna. 
    Since 2011, he has been with the Swiss Federal Institute of Technology, Lausanne, Switzerland, where he is Full Professor and the Chair of the Distributed Electrical Systems Laboratory. 
    His research interests focus on power systems with particular reference to real-time monitoring and operational aspects, power system protections, dynamics and transients. 
    Dr. Paolone’s most significant contributions are in the field of PMU-based situational awareness of active distribution networks (ADNs) and in the field of exact, convex and computationally-efficient methods for the optimal planning and operation of ADNs. 
    Dr. Paolone is Fellow of the IEEE and was the founder Editor-in-Chief of the Elsevier journal Sustainable Energy, Grids and Networks.
\end{IEEEbiography}

==> Sections/CIDER_Models.tex <==
% Reference calculation
\section{Extended Library of Resource Models}
\label{sec:cider:lib-rsc}

This section introduces the changes in the library of resource models, as compared to \cite{jrn:2020:kettner-becker:HPF-2} and \cite{jrn:2022:becker}, that are needed in order to derive the \HSS models of the \CIDER[s].
Specifically, three types of \CIDER[s] are considered for \HSA in this paper: (i) the grid-forming \CIDER that models only \AC-side characteristics, (ii) the grid-following \CIDER that models only \AC-side characteristics (both introduced in \cite{jrn:2020:kettner-becker:HPF-2}), and (iii) the grid-following \CIDER that includes the modelling of the \DC side (proposed in \cite{jrn:2022:becker}).
The modelling of the internal response (i.e., power hardware, control software and coordinate transformations) stays unchanged.
The difference as opposed to the \CIDER models previously introduced is the representation of the reference calculation as a small-signal model.
This applies to both of the grid-following \CIDER[s], namely the reference calculation being the PQ law.

\begin{figure}[t]
    \centering
    % \includegraphics[width=0.9\linewidth]{Figures/CIR.pdf}
    \input{Figures/Resource_Schematic}
    \caption
    {%
        Block diagram of the generic state-space model of \CIDER[s].
        Power hardware $\pwr$, control software $\ctrl$, and grid $\grd$ are interfaced via coordinate transformations $\tau_{\cdot|\cdot}$.
        The reference calculation $\mathbf{r}(\cdot,\cdot)$ may be either linear (i.e., for $\mathit{Vf}$ control) or nonlinear (i.e., for $\mathit{PQ}$ control).
        The other blocks of the model are exactly linear (i.e., \LTP systems and \LTP transforms).
    }
    \label{fig:CIDER:model}
\end{figure}

\subsection{Reference Calculation of the Grid-Following CIDERs}

In grid-following \CIDER[s], the reference angle $\theta$ needed for the \cmpDQ~transform is provided by a synchronization unit, usually a \emph{Phase-Locked Loop} (\PLL).
The reference current $\IT^*_{\grd,\cmpDQ}$ is computed in order to track the power setpoint $S_\spt=P_\spt+jQ_\spt$ at the fundamental frequency.
In the vast majority of cases, synchronization units in general, and \PLL[s] in particular, are designed to lock to the fundamental positive-sequence component of the grid voltage (e.g., \cite{Bk:Teodorescu:2011}).
As a consequence, the grid current reference is calculated purely based on the $\cmpD$-component of the grid voltage:
\begin{equation}
	\IT^*_{\grd,\cmpDQ}(t)
	\approx  
	\begin{bmatrix}
		 \frac{1}{v_{\grd,\cmpD}(t)} & 0\\
		0 &  \frac{1}{v_{\grd,\cmpD}(t)}
	\end{bmatrix}
	\begin{bmatrix}
		P_\spt\\
		Q_\spt
	\end{bmatrix}
	\label{eq:ref:following:simplified}
\end{equation}

As required by power quality standards (e.g., \cite{Std:BSI-EN-50160:2000}), the grid voltages have to be maintained balanced and sinusoidal within specified limits.
Under these conditions, it reasonable to assume the following.
\begin{Hypothesis}\label{hyp:rsc:follower:harms}
	The time-variant signal content of $v_{\grd,\cmpD}(t)$, as given by $\xi_\cmpD(t)$ below, is low:
	\begin{alignat}{2}
		v_{\grd,\cmpD}(t)
		&=      V_{\grd,\cmpD,0}(1+\xi_\cmpD(t)),~
		&       \Abs{\xi_\cmpD(t)}
		&\ll    1
	\end{alignat}
    where $V_{\grd,\cmpD,0}$ is the Fourier coefficient of $v_{\grd,\cmpD}(t)$ at $h=0$.
\end{Hypothesis}

% HSA - small signal model
\subsubsection{Small-Signal Model of the Reference Calculation}
For the representation of the reference calculation within the \HSS model of the \CIDER, the format introduced in Part~I of this paper in (12) is employed.
To this end, one needs to derive the coefficient matrices $	\hat{\mathbf{R}}_{\refr}$ and $\hat{\mathbf{R}}_{\spt}$ originating from the Taylor expansion in time domain, as well as the shift of the origin $\hat{\bar{\mathbf{W}}}_{\ctrl}$.
Rewrite \eqref{eq:ref:following:simplified} in terms of the \CIDER variables:
\begin{align}
	\mathbf{w}_{\ctrl}(t)
	&=\frac{1}{\mathbf{w}_\refr(t)} \mathbf{w}_\spt(t)
\end{align}
Then, the coefficients for the small-signal model of \eqref{eq:ref:following:simplified} for the operating point $\mathbf{\bar{w}}_\refr(t)$ and a general power setpoint $\mathbf{\bar{w}}_\spt(t)$ are given by
\begin{align}
    \mathbf{\bar{w}}_{\ctrl}(t)
	&=\frac{1}{\mathbf{\bar{w}}_\refr(t)} \mathbf{\bar{w}}_\spt(t)
    \label{eq:refcalc:w_k}
    \\
	\mathbf{R}_{\refr}(t)
	&=-\left(\frac{1}{\mathbf{\bar{w}}_\refr(t)}\right)^2 \mathbf{\bar{w}}_\spt(t)
     \label{eq:refcalc:r_refr}
     \\
		\mathbf{R}_{\spt}(t)
	&=\frac{1}{\mathbf{\bar{w}}_\refr(t)}
    \label{eq:refcalc:r_spt}
\end{align}
From this, the harmonic-domain quantities $\hat{\mathbf{W}}_{\ctrl}$, $\hat{\mathbf{R}}_{\refr}$, and $\hat{\mathbf{R}}_{\spt}$ are derived by means of the Teoplitz theory.
%
% ++++++++++
% Nonlinear
%
\subsubsection{Nonlinear Approximation of the Reciprocal of the Grid Voltage}
% In order to derive the \HSS model of the \CIDER, the Fourier coefficients of coefficient matrices in \eqref{eq:refcalc:w_k}--\eqref{eq:refcalc:r_spt} are needed.
% Unfortunately, the exact expressions that relate the Fourier coefficients of the reciprocal $\mathbf{\bar{w}}^{-1}_{\refr}$ (i.e., $v^{-1}_{\grd,\cmpD}$) and those of $\mathbf{\bar{w}}_{\refr}$ (i.e., $v_{\grd,\cmpD}$) are complicated \cite{Jrn:Edrei:1953}, and their evaluation is computationally intensive.
% However, taking advantage of \cref{hyp:rsc:follower:harms}, a Taylor expansion can be employed.
Similar to the derivations of the reference calculation used in the \HPF in \cite{jrn:2020:kettner-becker:HPF-2}, the reciprocal of $\mathbf{\bar{w}}_\refr(t) = \bar{v}_{\grd,\cmpD}(t)$ can be approximated by a Taylor expansion.
In this respect, the following hypothesis is made:
\begin{Hypothesis}\label{hyp:rsc:follower:approx}
	For the calculation of the reference current in the grid-following \CIDER[s], the reciprocal of the grid voltage can be approximated by a  Taylor series of order $n$:
	\begin{equation}
		\frac{1}{\bar{v}_{\grd,\cmpD}(t)}
		\approx \frac{1}{\bar{V}_{\grd,\cmpD,0}}\sum_n(-1)^n\xi_\cmpD^{n}(t)
	\end{equation}
	where the Fourier series of $\xi_\cmpD(t)$ is described by
	\begin{equation}
	\xi_{\cmpD}(t) = \sum_{h\neq0}\frac{\bar{V}_{\grd,\cmpD,h}}{\bar{V}_{\grd,\cmpD,0}}\Exp{jh2\pi f_1 t}
	\end{equation}
\end{Hypothesis}
\noindent
Employing this Taylor expansion, one can approximate the matrix in \eqref{eq:ref:following:simplified} by $\boldsymbol{\Psi}^{(n)}(t)$
\begin{equation}
\boldsymbol{\Psi}^{(n)}(t)
= \frac{1}{\bar{V}_{\grd,\cmpD,0}}	\sum_n(-1)^n	\boldsymbol{\Xi}_\cmpD^{n}(t)
\label{eq:ref:td:nth-order}
\end{equation}
where
\begin{align}
	\boldsymbol{\Xi}_\cmpD(t) = \diag(\mathbf{1}_2)\xi_\cmpD(t)
\end{align}

Transforming \eqref{eq:ref:td:nth-order} to the harmonic domain gives
\begin{align}
\hat{\mathbf{\Psi}} ^{(n)}=  \frac{1}{\bar{V}_{\grd,\cmpD,0}}\sum_n(-1)^n\hat{\boldsymbol{\Xi}}_{\cmpD}^{n}
\label{eq:ref:hd:nth-order}
\end{align}
where $\diag(\mathbf{1})$ is a matrix of suitable size, composed of ones, and $\hat{\boldsymbol{\Xi}}_{\cmpD}$ describes the Toeplitz matrix built from the Fourier coefficients of $\mathbf{\Xi}_{\cmpD}(t)$.

Using a second-order Taylor expansion one obtains
\begin{align}
	\hat{\mathbf{\Psi}}^{(2)} =  \frac{1}{\bar{V}_{\grd,\cmpD,0}}\left(\diag(\mathbf{1})-\hat{\boldsymbol{\Xi}}_{\cmpD}+\hat{\boldsymbol{\Xi}}_{\cmpD}^2\right)
\end{align}
The impact of the order of the expansion on the accuracy of the \CIDER model was investigated in \cite{ths:2024:becker} Chapter~3.
It is shown that the second order expansion of the reference calculation provides good accuracy of the \HSS model as validated through \emph{Time-Domain Simulations} (\TDS).
Notbaly, expansions of higher order can easily be obtained using \eqref{eq:ref:hd:nth-order} with suitable $n$.
% The impact of the order of the expansion on the \CIDER's grid response can be found in Chapter~3 of \cite{ths:2024:becker}.
Note that the approximation of the reciprocial of the grid voltage is a nonlinear function of the Fourier coefficients of the grid voltage.

% In general, one would expect that the nonlinear approximation of the reference calculation performs better than the small-signal model.
% However, if both models are evaluated at the operating point (i.e., with zero deviation from it), they will yield the same results.


==> Tables/Thevenin_Parameters_Resource.tex <==
{
	
	\renewcommand{\arraystretch}{1.1}
	
	\begin{tabular}{ccl}
		\hline
		Parameter
		&   Resource
		&   Description
		\\
		&   Validation
		\\
		\hline
		$V_{n}$
		&   230\,V-\RMS
		&   Nominal voltage 
		\\
		$S_{\mathit{sc}}$
		&   267\,kW
		&   Short-circuit power
		\\
		$\Abs{Z_{\mathit{sc}}}$
		&   195\,m$\Omega$
		&   Short-circuit impedance
		\\
		$R_{\mathit{sc}}/X_{\mathit{sc}}$
		&   6.207
		&   Resistance-to-reactance ratio
		\\
		\hline
	\end{tabular}
}

==> Tables/Thevenin_Parameters_System.tex <==
{
	
	\renewcommand{\arraystretch}{1.1}
	
	\begin{tabular}{cccl}
		\hline
		Parameter
		&   System
		&   Description
		\\
		&   Validation
		\\
		\hline
		$V_{n}$
		&   230\,V-\RMS
		&   Nominal voltage 
		\\
		$S_{\mathit{sc}}$
		&   3.85\,MW
		&   Short-circuit power
		\\
		$\Abs{Z_{\mathit{sc}}}$
		&   13.7\,m$\Omega$
		&   Short-circuit impedance
		\\
		$R_{\mathit{sc}}/X_{\mathit{sc}}$
		&   0.271
		&   Resistance-to-reactance ratio
		\\
		\hline
	\end{tabular}
}
